A Ranking-based, Balanced Loss Function Unifying Classification and Localisation in Object Detection

We propose average Localisation-Recall-Precision (aLRP), a unified, bounded, balanced and ranking-based loss function for both classification and localisation tasks in object detection. aLRP extends the Localisation-Recall-Precision (LRP) performance metric (Oksuz et al., 2018) inspired from how Average Precision (AP) Loss extends precision to a ranking-based loss function for classification (Chen et al., 2020). aLRP has the following distinct advantages: (i) aLRP is the first ranking-based loss function for both classification and localisation tasks. (ii) Thanks to using ranking for both tasks, aLRP naturally enforces high-quality localisation for high-precision classification. (iii) aLRP provides provable balance between positives and negatives. (iv) Compared to on average $\sim$6 hyperparameters in the loss functions of state-of-the-art detectors, aLRP Loss has only one hyperparameter, which we did not tune in practice. On the COCO dataset, aLRP Loss improves its ranking-based predecessor, AP Loss, up to around $5$ AP points, achieves $48.9$ AP without test time augmentation and outperforms all one-stage detectors. Code available at: https://github.com/kemaloksuz/aLRPLoss .

==> sections/deleted.tex <==
\comment{
\begin{table}[t]
    \centering
    \caption{Loss functions of the SOTA methods require tuning several hyperparameters. FL: Focal Loss, CE: Cross Entropy, SL1: Smooth L1, H: Hinge Loss. See the Supp. Mat. for descriptions of the required hyper-parameters.}
    \label{tab:Hyperparameters}
    \begin{tabular}{|l|l|c|l|}\hline
         Method&$\mathcal{L}$ & \multicolumn{2}{c|}{Number of Hyper-parameters \& Comments\quad} \\ \hline \hline
        AP Loss\cite{APLoss}&AP Loss+$\alpha$ SL1&3&-- \\ \hline
        Focal Loss\cite{FocalLoss}&FL+ $\alpha$ SL1&4&-- \\ \hline
        FCOS\cite{FCOS}&FL+$\alpha$ IoU+$\beta$ CE&4&Has an additional centerness branch\\  \hline
        DR Loss\cite{DRLoss}&DR Loss+$\alpha$ SL1&5&--\\ \hline
        FreeAnchor\cite{FreeAnchor}& $\alpha \log(\max( e^\text{CE} \times e^{\beta \text{SL1}}))$+$\gamma$ FL&8&Learns assignment via loss function \\\hline
        Faster R-CNN\cite{FasterRCNN}&CE+$\alpha$ SL1+$\beta$CE+$\gamma$ SL1&9&Two stage, sampling parameters to be tuned\\ \hline
        Center Net\cite{CenterNet}&FL+FL+$\alpha$ L2+$\beta$ H+$\gamma$ (SL1+SL1)&10&Uses more losses to learn centers\&corners  \\ \hline \hline
        Ours&aLRP Loss&1&Parameter from AP Loss. No tuning required.\\ \hline         
    \end{tabular}
\end{table}
}

\comment{
\begin{figure}
\begin{floatrow}
\capbtabbox{%
    \setlength{\tabcolsep}{0.1em}
    \caption{Effect of correlating the ranks of the classification scores and the ranks of the IoUs.}
    \label{tab:correlationEffect}
    \begin{tabular}{|l|c|c|c|c|c|} \hline
        $\mathcal{L}$&$\mathrm{AP}$&$\mathrm{AP_{50}}$&$\mathrm{AP_{75}}$&$\mathrm{AP_{90}}$&$\Bar{\sigma}$\\ \hline
        aLRP Loss&$38.7$&$58.1$&$40.6$&$17.4$&$0.48$\\ 
        %\multicolumn{2}{|c|}{aLRP L. w DIoU+w ASB}&$38.7$&$58.4$&$40.0$&$17.2$&$0.46$\\ 
        \hline
        Lower Bound&$28.6$&$58.1$&$23.6$&$5.6$&$-1.00$\\ 
        Upper Bound&$48.1$&$58.1$&$51.9$&$33.9$&$1.00$\\ 
        \hline
    \end{tabular}

}{}
\ffigbox[\FBwidth]{%
  \centering 
  \includegraphics[width=0.45\textwidth]{NIPS2020/figures/LossPlot.pdf}%
}{%
     \caption{The values of the aLRP Loss and its components during training. The regression component is adaptively balanced.
    \label{fig:LossPlot}
    }%
}
\end{floatrow}
\end{figure}
}

\comment{
\begin{figure}
\begin{floatrow}
\capbtabbox{%
    \setlength{\tabcolsep}{0.1em}
    \caption{Comparison of different loss function combinations on COCO \textit{minival}. The backbone is ResNet-50 and image scale is $500$.  ASB: Adaptive Self Balance, SL1:Smoooth L1}
    \label{tab:minival}
    \begin{tabular}{|l|c|c|c|c|c|c|c|} \hline
        $\mathcal{L}$&$\mathcal{L}_c$ Ranking Based&$\mathcal{L}_r$ Ranking Based&$\mathrm{AP}$&$\mathrm{AP_{50}}$&$\mathrm{AP_{75}}$&$\mathrm{AP_{90}}$&$\Bar{\sigma}$\\ \hline
        Focal Loss+SL1& & &$36.3$&$56.9$&$38.3$&$12.2$&$0.44$\\ \hline
        AUC Loss+SL1&\checkmark& &$25.5$&$44.9$&$26.0$&-&-\\ 
        %Focal L. \cite{FocalLoss}$^*$&SL1 L.\cite{FastRCNN}&$28.3$&$45.7$&$29.5$&$8.7$&\\        
        AP Loss+SL1&\checkmark& &$35.5$&$58.0$&$37.0$&$9.0$&$0.45$\\ 
        AP Loss+IoU&\checkmark& &$36.3$&$57.9$&$37.9$&$11.8$&$0.44$\\ 
        AP Loss+GIoU&\checkmark& &$36.5$&$58.1$&$38.1$&$11.9$&$0.45$\\ 
        %AP L. \cite{APLoss}&DIoU L.\cite{DIoULoss}&$36.6$&$58.3$&$38.5$&$11.9$&$0.45$\\ 
        \hline 
        aLRP L. w IoU&\checkmark&\checkmark&20&May& & &\\ 
        aLRP L. w IoU \& ASB&\checkmark&\checkmark&$38.7$&$58.1$&$40.6$&$17.4$&$0.48$\\ 
        aLRP L. w GIoU\& ASB&\checkmark&\checkmark&$38.9$&$58.5$&$40.4$&$17.4$&$0.48$\\ 
        %\multicolumn{2}{|c|}{aLRP L. w DIoU+w ASB}&$38.7$&$58.4$&$40.0$&$17.2$&$0.46$\\ 
        \hline
        %\multicolumn{2}{|c|}{aLRP L.(Lower Bound)}&$28.6$&$58.1$&$23.6$&$5.6$&$-1.00$\\ 
        %\multicolumn{2}{|c|}{aLRP L.(Upper Bound)}&$48.1$&$58.1$&$51.9$&$33.9$&$1.00$\\ 
        %\hline
    \end{tabular}

}{}
\ffigbox[\FBwidth]{%
  \centering 
  \includegraphics[width=0.38\textwidth]{NIPS2020/figures/LossPlot.pdf}%
}{%
     \caption{The values of the aLRP Loss and its components during training. The regression component is adaptively balanced.
    \label{fig:LossPlot}
    }%
}
\end{floatrow}
\end{figure}

}


\comment{
\begin{table}[t]
    \centering
%    \scriptsize 
    %\renewcommand{\arraystretch}{1.3}
    \caption{Performance comparison of the state-of-the art detectors on COCO \textit{test-dev}.Models with * are using Soft NMS \cite{SoftNMS} and flip augmentation during inference. R: ResNet, X:ResNeXt, H:HourglassNet, D:DarkNet.}
    \label{tab:testdev}
    \setlength{\tabcolsep}{0.2em}
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|} \hline
%        & & &VOC07&VOC12&\multicolumn{6}{c|}{COCO}\\\cline{4-11}
        Method&Backbone&Tra.Size&Test Size&Tra.Epoch&$\mathrm{AP}$&$\mathrm{AP_{50}}$&$\mathrm{AP_{75}}$&$\mathrm{AP_{S}}$ &$\mathrm{AP_{M}}$&$\mathrm{AP_{L}}$ \\ 
        \hhline{===========}
        \textit{One-Stage Methods}& & & & & & & & & &\\
        RetinaNet\cite{FocalLoss}&R-101&$500$&$500$&$\sim12$&$34.4$&$53.1$&$36.8$&$14.7$&$38.5$&$49.1$\\
        RefineDet\cite{AnchorRefine}&R-101&$512$&$512$&$\sim110$&$36.4$&$57.5$&$39.5$&$16.6$&$39.9$&$51.4$\\
        EFGRNet\cite{EnrichedFeatureGuided}&R-101&$512$&$512$&$160$&$39.0$&$58.8$&$42.3$&$17.8$&$43.6$&$54.5$\\ 
        HSD\cite{HierarchicalShotDet}&R-101&$512$&$512$&$160$&$40.2$&$59.4$&$44.0$&$20.0$&$44.4$&$54.9$\\
        CenterNet\cite{CenterNet}&H-52&$512$&orig.&$\sim200$&$41.6$&$59.4$&$44.2$&$22.5$&$43.1$&$54.1$\\
        RetinaNet\cite{FocalLoss}&R-101&$800$&$800$&$\sim18$&$39.1$& $59.1$ &$42.3$&$21.8$&$42.3$&$50.2$\\        
        FCOS\cite{FCOS}&R-101&$640,800$&$800$&$\sim24$&$41.5$&$60.7$&$45.0$&$24.4$&$44.8$&$51.6$\\
        FreeAnchor\cite{FreeAnchor}&R-101&$640,800$&$800$&$\sim24$&$43.1$&$62.2$&$46.4$&$24.5$&$46.1$&$54.8$ \\ \hline
        HSD\cite{HierarchicalShotDet}&X-101&$512$&$512$&$160$&$41.9$&$61.1$&$46.2$&$21.8$&$46.6$&$57.0$\\ 
        CornerNet\cite{CornerNet}$^*$&H-104&$511$&orig.&$\sim210$&$40.5$&$56.5$&$43.1$&$19.4$&$42.7$&$53.9$\\
        ExtremeNet\cite{ExtremeNet}$^*$&H-104&$511$&orig.&$\sim100$&$40.2$&$55.5$&$43.2$&$20.4$&$43.2$&$53.1$\\
        CenterNet\cite{CenterNet}$^*$&H-104&$511$&orig.&$\sim200$&$44.9$&$62.4$&$48.1$&$25.6$&$47.4$&$57.4$\\          
        RetinaNet\cite{FocalLoss}&X-101&$800$&$800$&$\sim18$&$40.8$&$61.1$&$44.1$&$24.1$&$44.2$&$51.2$\\
        FCOS\cite{FCOS}&X-101&$640,800$&$800$&$\sim24$&$43.2$&$62.8$&$46.6$&$26.5$&$46.2$&$53.3$\\ 
        FreeAnchor\cite{FreeAnchor}&X-101&$640,800$&$800$&$\sim24$&$44.9$&$64.3$&$48.5$&$26.8$&$48.3$&$55.9$\\
        \hhline{===========}
        \textit{Ranking Losses}& & & & & & & & & &\\  
        DRLoss \cite{DRLoss}&R-50&$500$&$500$&$12$&$34.5$&$52.6$&$36.6$&$14.7$ &$36.9$&$48.9$\\            
        AP Loss\cite{APLoss}&R-101&$512$&$500$&$100$&$37.4$&$58.6$&$40.5$&$17.3$&$40.8$&$51.9$\\
        DR Loss\cite{DRLoss}&R-101&$640,800$&$800$&$24$&$41.7$&$60.9$&$44.8$&$23.5$&$44.9$&$53.1$\\ 
        AP Loss\cite{APLoss}&R-101&$800$&$800$&$100$&$40.8$&$63.7$&$43.7$&$25.4$&$43.9$&$50.6$\\
        DR Loss\cite{DRLoss}&X-101&$640,800$&$800$&$24$&$43.1$&$62.8$&$46.4$&$25.6$&$46.2$&$54.0$\\        
        \hhline{===========}
        \textit{Multi-Task L. in OD}& & & & & & & & & &\\
        LapNet\cite{LapNet}&D-53&$512$&$512$&$\sim120$&$37.6$&$55.5$&$40.4$&$17.6$&$40.5$&$49.9$\\ 
        Retina+PISA\cite{PrimeSample}&R-101&$800$&$800$&$\sim12$&$40.8$&$60.5$&$44.2$&$23.0$&$44.2$&$51.4$\\
        \hhline{===========}
        \textit{Ours}& & & & & & & & & &\\
        aLRP Loss&R-50&$512$&$500$&$160$&24&May& & & &  \\
        aLRP Loss&R-101&$512$&$500$&$160$&$41.5$&$61.3$&$43.8$&$21.2$&$44.9$&$56.7$\\  
        aLRP Loss&X-101&$512$&$500$&$160$&24&May&  &  &  &  \\
%        aLRP Loss&R-101&$800$&$800$&$24$& &  &  &  &  &  \\        
%        aLRP Loss&X-101&$800$&$800$&$24$&  & & &  &  &  \\
        aLRP Loss&R-101&$800$&$800$&$100$&? & &  &  &  &  \\        
        aLRP Loss&X-101&$800$&$800$&$100$&31&May & &  &  &  \\        
%        aLRP Loss&X-101&$512$&Multi& &  &  & &  &  &  \\    
        \hline

%        \textit{Multi-Scale}& & & & & & & & & &\\
%        RefineDet \cite{AnchorRefine}& ResNet-101 &N/A& $xx$ & $xx$ & $41.8$ & $62.9$ & $45.7$ & $25.6$ & $45.1$ & $54.1$\\ 
%        RetinaNet+AP-Loss \cite{APLoss} & ResNet-101 & N/A& $84.9$ & $84.5$ & $42.1$ & $63.5$ & $46.4$ & $25.6$ & $45.0$ & $53.9$ \\        
%        RetinaNet+DR Loss \cite{DRLoss} & ResNet-101&N/A& $xx$ & $xx$ & $43.4$ & $62.1$ & $47.0$ & $26.7$ & $46.1$ & $55.0$  \\     
%        aLRP Loss (ours) & ResNet-101 & N/A & &  & &  &  &  &  &  \\        
%        \hline        
    \end{tabular}
\end{table}
}
